A Note on Coloring $(4K_1, C_4, C_6)$-free graphs with a $C_7$

Even-hole-free graphs are a graph class of much interest. Foley et al. [Graphs Comb. 36(1): 125-138 (2020)] have recently studied $(4K_1, C_4, C_6)$-free graphs, which form a subclass of even-hole-free graphs. Specifically, Foley et al. have shown an algorithm for coloring these graphs via bounded clique-width if they contain a $C_7$. In this note, we give a simpler and much faster algorithm via a more restrictive graph parameter, neighborhood diversity.

==> macros/appHandler.tex <==
%%%% Appendix Handler %%%%
\usepackage{etoolbox}

\newcommand{\sv}[1]{#1}
\newcommand{\lv}[1]{#1}

\newcommand{\appendixText}{}

\newcommand{\toappendix}[1]{\gappto{\appendixText}{{#1}}}
%\newcommand{\toappendix}[1]{#1}

\newcommand{\appmark}{$\star$}


==> macros/theorems.tex <==
%\usepackage{amsthm}
%\usepackage{mathtools}
%%% theorem, definition an so on %%%
%\theoremstyle{plain}
%\newtheorem{theorem}{Theorem}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem*{fact*}{Fact}

%\theoremstyle{definition}
%\newtheorem{definition}{Definition}
%\newtheorem*{example*}{Example}

% Reptheorem\textsc{
\makeatletter
\newtheorem*{rep@theorem}{\rep@title}
\newcommand{\newreptheorem}[2]{%
\newenvironment{rep#1}[1]{%
 \def\rep@title{#2 \ref{##1}}%
 \begin{rep@theorem}}%
 {\end{rep@theorem}}}
\makeatother

\newreptheorem{theorem}{Theorem}
%\newreptheorem{corollary}{Corollary}
\newreptheorem{lemma}{Lemma}
%\newreptheorem{proposition}{Proposition}}

%\theoremstyle{remark}
%\newtheorem{observation}{Observation}
%\newtheorem{claim}{Claim}
%\newtheorem*{claim*}{Claim}
%\newtheorem*{remark}{Remark}



==> macros/todo.tex <==
\usepackage[textwidth=20mm,obeyFinal,colorinlistoftodos]{todonotes}
\newcommand{\mytodo}[2]{\todo[size=\tiny, color=#1!50!white]{#2}\xspace}
\newcommand{\myinlinetodo}[2]{\todo[size=\small, color=#1!50!white, inline]{#2}\xspace}
\newcommand{\mmcom}[1]{\mytodo{red}{#1}}
\newcommand{\sebastian}[1]{\mytodo{green}{#1}}
\newcommand{\sebastianinline}[1]{\myinlinetodo{green}{#1}}
\newcommand{\martin}[1]{\mytodo{blue}{#1}}
\newcommand{\martininline}[1]{\myinlinetodo{blue}{#1}}
\newcommand{\cornelius}[1]{\mytodo{yellow}{#1}}
